Tiny Titans: Can Smaller Large Language Models Punch Above Their Weight in the Real World for Meeting Summarization?

Large Language Models (LLMs) have demonstrated impressive capabilities to solve a wide range of tasks without being explicitly fine-tuned on task-specific datasets. However, deploying LLMs in the real world is not trivial, as it requires substantial computing resources. In this paper, we investigate whether smaller, compact LLMs are a good alternative to the comparatively Larger LLMs2 to address significant costs associated with utilizing LLMs in the real world. In this regard, we study the meeting summarization task in a real-world industrial environment and conduct extensive experiments by comparing the performance of fine-tuned compact LLMs (e.g., FLAN-T5, TinyLLaMA, LiteLLaMA) with zero-shot larger LLMs (e.g., LLaMA-2, GPT-3.5, PaLM-2). We observe that most smaller LLMs, even after fine-tuning, fail to outperform larger zero-shot LLMs in meeting summarization datasets. However, a notable exception is FLAN-T5 (780M parameters), which performs on par or even better than many zero-shot Larger LLMs (from 7B to above 70B parameters), while being significantly smaller. This makes compact LLMs like FLAN-T5 a suitable cost-efficient solution for real-world industrial deployment.

==> table.tex <==
\begin{table*}
\centering
\tiny
%\setlength{\tabcolsep}{4pt} 
\begin{tabular}{l|l|cccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{\textbf{Dataset}} \\ \cmidrule(r){3-6}  
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Type}} &  \multicolumn{4}{c}{\textbf{MeetingBank}}  \\
\cmidrule(r){3-6} 

\multicolumn{1}{c}{} & \multicolumn{1}{c}{}
%& \textbf{R-1} &  \textbf{R-2} &   \textbf{R-L} &   \textbf{B-S} 
& \textbf{R-1} &  \textbf{R-2} &   \textbf{R-L} &   \textbf{B-S}  \\
\midrule

GPT-3.5     & chapter (concat)
 & 22.78 &  9.06 & 16.42 & 54.76 
 \\
GPT-3.5      & chapter (resummarize) 
& 24.86 &  9.33 & 17.52  & 55.95 
 \\
GPT-3.5     & chapter (rewrite)     
 & 24.71 &  9.26 & 17.31 & 55.93 
  &                      {7.55}&                \textbf{16.29} &                 57.25 \\
GPT-3.5     & truncation       
& 25.63 &  9.90  & 18.31  & 56.24 
 \\
\midrule
GPT-4       & chapter (concat) 
& 25.76	& 10.61	& 18.29	& 57.58   \\



GPT-4        & chapter (resummarize) 
 & \textbf{27.02}    & 10.85 & \textbf{18.93} & \textbf{57.78} 
 \\

GPT-4       & chapter (rewrite)     
& 26.01 & 10.68 & 18.54 & 57.54 
\\
GPT-4       & truncation      
 & 26.82  & 10.87 & 18.68 & 57.75 
 \\
\midrule
 
   PaLM-2      & chapter (concat)
   & 22.01    &  9.34 & 16.68 & 53.65 
 \\
 PaLM-2       & chapter (resummarize) 
& 23.02 &  9.81 & 17.52 & 53.95 
 \\

PaLM-2      & chapter (rewrite)   
& 22.51 &  9.56 & 17.12 & 53.87 
\\
PaLM-2      & truncation      
 & 20.86 &  9.67 & 16.79 & 52.08 
\\
\midrule

LLaMA-2-13b & chapter (concat) 
& 13.44 &  7.76 & 10.77 & 51.52 
 \\


LLaMA-2-13b  & chapter (resummarize) 
& 26.61 & 10.53 & 18.86 & 56.82 
 \\

 LLaMA-2-13b & chapter (rewrite)     
 & 18.66 &  9.63 & 14.29  & 52.84 
\\
LLaMA-2-13b & truncation      
& 24.55 & 11.03 & 17.82 & 56.05 
 \\
\midrule


LLaMA-2-7b  & chapter (concat) 
& 13.49 &  7.66 & 10.73 & 51.59 
 \\

 LLaMA-2-7b   & chapter (resummarize)
 & 26.38 & 11.01 & 18.77 & 57.83 
 \\
 
 LLaMA-2-7b  & chapter (rewrite)    
& 20.17 &  9.41  & 14.92 & 54.23 \\


 LLaMA-2-7b  & truncation       
 & 24.75 & \textbf{11.08} & 17.95 & 56.49 \\

\bottomrule

\end{tabular}
\caption{\small{Performance of LLMs on the QMSUM (Filtered), AMI, and ICSI Datasets.}}
\label{tab:results}
\end{table*}

